Efficient Parallel Execution of Blockchain Transactions Leveraging Conflict Specifications

Parallel execution of smart contract transactions in large multicore architectures is critical for higher efficiency and improved throughput. The main bottleneck for maximizing the throughput of a node through parallel execution is transaction conflict resolution: when two transactions interact with the same data, like an account balance, their order matters. Imagine one transaction sends tokens from account A to account B, and another tries to send tokens from account B to account C. If the second transaction happens before the first one, the token balance in account B might be wrong, causing the entire system to break. Conflicts like these must be managed carefully, or you end up with an inconsistent, unusable blockchain state. Traditional software transactional memory (STM) has been identified as a possible abstraction for the concurrent execution of transactions within a block, with Block-STM pioneering its application for efficient blockchain transaction processing on multicore validator nodes. This paper presents a parallel execution methodology that leverages conflict specification information of the transactions for block transactional memory (BTM) algorithms. Our experimental analysis, conducted over synthetic transactional workloads and real-world blocks, demonstrates that BTMs leveraging conflict specifications outperform their plain counterparts on both EVM and MoveVM. Our proposed BTM implementations achieve up to 1.75x speedup over sequential execution and outperform the state-of-the-art Parallel-EVM (PEVM) execution by up to 1.33x across synthetic workloads.

==> new_results.tex <==
\section{New Historical Block Results: Best, Average, and Worst Case}

\paragraph*{Best Case - 17873654}
The block contains 136 transactions, including 435 contract internal transactions, with the majority being smart contract transactions. Approximately 38\% of the transactions are independent, and the longest conflict chain spans 50 transactions. In this scenario, \saSupraSTM{} achieves the best performance among all evaluated approaches, delivering a maximum speedup of 1.98× compared to sequential execution. \saBlockSTM{} performance is similar to that of \PEVM{}.


\paragraph*{Average Case - 17873668}

The block consists of 132 transactions and includes 249 internal contract calls. Approximately 48\% of the transactions are independent, while the longest conflict chain spans 33 transactions. Most of the transaction are smart contract interactions. All approaches deliver comparable performance, with \saSupraSTM{} achieving a maximum speedup of 1.65$\times$ over sequential execution.

\paragraph*{Worst Case - 17873752}
This is a large block containing 1189 transactions, of which 1129 are native ETH transfers. The available parallelism is minimal, with only 4\% of transactions being independent, and the longest conflict chain reaching 1104 transactions. This represents the worst-case scenario for \saSupraSTM{}, as it must process the dependent native ETH transfers sequentially. Dependencies are added for these transactions, and they are subsequently handled through lazy updates, introducing additional overhead compared to sequential execution. For both \saBlockSTM{} and \PEVM{}, performance is comparable to sequential execution due to the sequential post-processing of native ETH transfers using lazy updates.
\begin{table}[htbp]
    \caption{Benchmark Results on Historical Ethereum Blocks}
    \label{tab:transposed-benchmark}
    \centering
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{|r|l|c|c|c|c|c|c|c|c|c|c|}
            \hline
            \multicolumn{2}{|c|}{\textbf{Metric}} &
            \multicolumn{2}{c|}{\textbf{Recent Blocks}} &
            \multicolumn{2}{c|}{\textbf{Ethereum 2.0}} &
            \multicolumn{2}{c|}{\textbf{CryptoKitties}} &
            \multicolumn{4}{c|}{\textbf{Large Blocks}} \\
            \hline
            \multicolumn{2}{|c|}{} &
            \textbf{20320204} & \textbf{20320205} & \textbf{15537400} & \textbf{15537401} &
            \textbf{4605100} & \textbf{4605101} & \textbf{17873752} & \textbf{17873746} &
            \textbf{17873731} & \textbf{17873654} \\
            \hline

            \multirow{4}{*}{Block Stats}
                & Block Size              & 147      & 151      & 178      & 70       & 53       & 34       & 1189    & 897     & 914      & 136 \\
                \cline{2-12}
                & Native ETH Txns         & 40       & 50       & 14       & 9        & 11       & 15       & 1129    & 810     & 820      & 41 \\
                \cline{2-12}
                & \ERC{} Txns             & 50       & 57       & 6        & 0        & 6        & 8        & 21      & 25      & 36       & 18 \\
                \cline{2-12}
                & Smart Contract Txns     & 57       & 44       & 158      & 61       & 36       & 11       & 39      & 62      & 58       & 77 \\
            \hline

            \multirow{2}{*}{Analysis Phase}
                & Decompilation (sec)     & 15.57 s & 74.22 s & 120.63 s & 6.79 s  & 3.81 s  & 5.63 s  & 73.35 s & 15.63 s & 120.68 s & 11.31 s \\
                \cline{2-12}
                & Pre-processing (ms)     & 89.40   & 103.17  & 89.98    & 13.16   & 11.21   & 7.61    & 40.81   & 82.00   & 77.45    & 49.81 \\
            \hline

            \multirow{2}{*}{Conflict Set (Strong)}
                & Generation Time         & 76.91~µs & 78.58~µs & 113.02~µs & 36.85~µs & 17.86~µs & 17.62~µs & 2.53~ms & 2.29~ms & 2.62~ms & 66.25~µs \\
                \cline{2-12}
                & Specification Size      & 4180     & 6260     & 4531      & 1200     & 135      & 230      & 54155   & 56134   & 63559    & 1930 \\
            \hline

            \multirow{2}{*}{Conflict Set (Weak)}
                & Generation Time         & 92.60~µs & 70.73~µs & 26.59~µs & 15.16~µs & 19.47~µs & 17.52~µs & 2.60~ms & 2.43~ms & 2.58~ms & 45.89~µs \\
                \cline{2-12}
                & Specification Size      & 3972     & 5630     & 190      & 36       & 135      & 207      & 50706   & 53654   & 63590    & 1691 \\
            \hline

            \multirow{4}{*}{Avg Exec Time}
                & Sequential              & 8.34~ms  & 11.12~ms & 6.78~ms  & 1.43~ms  & 747.82~µs & 498.34~µs & 7.27~ms & 12.59~ms & 11.41~ms & 36.46~ms \\
                \cline{2-12}
                & \PEVM{}                    & 6.52~ms  & 6.80~ms  & 2.70~ms  & 1.14~ms  & 900.77~µs & 559.17~µs & 6.07~ms & 7.81~ms  & 6.61~ms  & 27.67~ms \\
                \cline{2-12}
                & \saSupraSTM{}              & 8.23~ms  & 6.54~ms  & 3.12~ms  & 1.21~ms  & 929.57~µs & 772.33~µs & 8.91~ms & 10.76~ms & 7.79~ms  & 19.14~ms \\
                \cline{2-12}
                & \saBlockSTM{}              & 6.50~ms  & 6.89~ms  & 2.61~ms  & 1.12~ms  & 922.27~µs & 532.96~µs & 5.89~ms & 7.91~ms  & 6.21~ms  & 27.55~ms \\
            \hline

        \end{tabular}%
    }
\end{table}

\paragraph*{Implementation Details}

In our project, we used REVM version 12.1.0 and compared our results against \PEVM{} version 0.1.0, specifically at commit hash \texttt{f0bdb21}. We leveraged the core data structures provided by \PEVM{} and implemented our own algorithms on top of them. In particular, we utilized a hash map to store the conflict set ($\Cset{}$), which allowed us to derive both the list of dependent transactions and the indegree of each transaction within the DAG.

For the \saBlockSTM{} evaluation, we determined transaction independence by checking whether a transaction’s $\Cset{}$ included all preceding transactions, ensuring it could execute without conflicts. In the case of integrated experiments, where we lacked complete specifications from the weak conflict analyzer, we adopted an optimistic execution strategy for transactions with incomplete or unknown specifications. While waiting for the set of dependencies to clear for conflicting transactions before scheduling them.


\section{Aptos Block Results: Best, Average, and Worst Case}

\paragraph*{Batch Transfer Good Case - $10^4$ Block Size}
Under low conflict conditions, parallel execution strategies show significant performance gains compared to sequential execution. The sequential baseline remains at 20445~ms, while \BSTM, \saSupraSTM{}, and \saBlockSTM{} reduce execution times to 1725~ms, 2606~ms, and 1692~ms respectively, all using 16 threads. \saBlockSTM{} delivers the best performance, achieving a 12$\times$ speedup over sequential execution. \BSTM follows closely, slightly outperforming \saSupraSTM{}. The results demonstrate that in low conflict environments, all STM-based strategies scale well, and \saBlockSTM{} is particularly effective.


\paragraph*{Batch Transfer Average Case - $10^4$ Block Size}
In the medium conflict scenario, the performance of all \STM{} variants degrades as contention increases, but still offers substantial gains over sequential execution. The execution time for sequential remains constant at 20445~ms, whereas \BSTM{}, \saSupraSTM{}, and \saBlockSTM{} report 5173~ms, 5288~ms, and 5096~ms, respectively. These figures represent approximately a 4$\times$ speedup over the sequential baseline. Notably, \saBlockSTM{} maintains a slight edge over the others even under increased contention, while \saSupraSTM{} and \BSTM{} perform comparably. This indicates that \STM{} frameworks still provide meaningful concurrency benefits even with moderate conflicts, though the margin narrows.


\paragraph*{Batch Transfer Worst Case - $10^4$ Block Size}
Under high conflict conditions, the benefits of parallel execution diminish drastically due to frequent contention and rollback overhead. The sequential time remains unchanged at 20445~ms, while \BSTM{}, \saSupraSTM{}, and \saBlockSTM{} show increased execution times of 24036~ms, 20476~ms and 20373~ms, respectively. Here, all \STM{} variants perform worse than sequential, with \BSTM{} suffering the most degradation. \saBlockSTM{} still marginally outperforms the others, but the overhead of conflict resolution outweighs the gains from concurrency. This illustrates that \STM{} strategies are sensitive to high conflict workloads and may require adaptive mechanisms or conflict avoidance strategies to remain efficient.


\paragraph*{P2P Good Case - $10^4$ Block Size}
Under low conflict conditions, all STM-based strategies show outstanding performance improvements over sequential execution. The sequential execution time is 4389~ms, while \BSTM{}, \saSupraSTM{}, and \saBlockSTM{} reduce this to 393~ms, 535~ms, and 387~ms, respectively. \saBlockSTM{} performs the best, achieving more than an 11$\times$ speedup, closely followed by \BSTM{}. Even the slowest among the \STM{} variants, \saBlockSTM{}, still achieves an 8$\times$ improvement. These results highlight that in low-contention P2P transaction workloads, \STM{} strategies, especially \saBlockSTM{} scale efficiently and effectively leverage parallelism.

\paragraph*{P2P Average Case - $10^4$ Block Size}
In a moderate conflict scenario, the \STM{} methods still provide substantial gains, though the performance advantage narrows due to increased contention. The sequential time remains 4389~ms, while \BSTM{}, \saSupraSTM{}, and \saBlockSTM{} take 1111~ms, 974~ms, and 1108~ms, respectively. Interestingly, \saSupraSTM{} slightly outperforms the other variants, marking a 4.5$\times$ speedup, while the others achieve 4$\times$ speedup. This indicates that even under moderate contention, STM-based execution maintains strong scalability, although performance benefits taper compared to low-conflict conditions.

\paragraph*{P2P Worst Case - $10^4$ Block Size}
With high conflict, performance degrades across all \STM{} systems, though not drastically worse than the sequential baseline. The sequential execution time is 4389~ms, while \BSTM{}, \saSupraSTM{}, and \saBlockSTM{} take 5190~ms, 3806~ms, and 4293~ms, respectively. Notably, \BSTM{} performs worse than sequential, showing the penalty of high rollback and synchronization overhead. However, \saSupraSTM{} remains faster than sequential, showing resilience under contention, and  \saBlockSTM{} is only marginally slower. These results emphasize that not all \STM{} systems are equally affected by high conflict.

\section{Diem Block Results: Best, Average, and Worst Case}

\paragraph*{Batch Transfer Good Case - $10^4$ Block Size}
In low-contention conditions, all \STM{} variants significantly outperform sequential execution (4551~ms). \saBlockSTM{} achieves the lowest latency at 236~ms, closely followed by \BSTM{} (249~ms) and \saSupraSTM{} (300~ms), yielding a ~19× speedup. These results indicate that batch transfers with minimal conflicts are highly amenable to speculative parallel execution.

\paragraph*{Batch Transfer Average Case - $10^4$ Block Size}
At moderate contention levels, \STM{} performance degrades due to increased transaction aborts but still provides notable improvements. \saSupraSTM{} leads with 823~ms, while \BSTM{} and \saBlockSTM{} report similar performance at 1017~ms and 1013~ms. The 4.5–5.5$\times$ speedup confirms that speculative execution remains beneficial for batch transfers under moderate conflict.

\paragraph*{Batch Transfer Worst Case - $10^4$ Block Size}
With high contention, speculative execution incurs significant coordination overhead. \saSupraSTM{} is the only strategy outperforming sequential, completing in 3589~ms. \BSTM{} and \saBlockSTM{} exceed the baseline, with execution times of 4753~ms and 4741~ms, respectively. This suggests that \saSupraSTM{’s} conflict resolution strategy is more resilient under heavy contention, making it more suitable for batch transfer workloads in adverse conditions.


\paragraph*{P2P Good Case - $10^4$ Block Size}
In low-contention P2P workloads, STM-based strategies deliver very high parallel efficiency. Both \BSTM{} and \saBlockSTM{} achieve 156~ms, while \saSupraSTM{} completes in 187~ms, resulting in an 21$\times$ speedup over sequential execution. This demonstrates that with minimal conflicts, speculative parallelism is highly effective for fine-grained P2P transaction patterns.


\paragraph*{P2P Average Case - $10^4$ Block Size}
Under moderate contention, performance benefits persist but diminish due to increased coordination overhead. \saSupraSTM{} leads at 535~ms, while \BSTM{} and \saBlockSTM{} follow closely at 659~ms and 672~ms, respectively. This represents a 5–6$\times$ improvement over sequential, showing that P2P workloads still scale well under moderate conflicts, particularly for \STM{} engines with efficient conflict resolution.

\paragraph*{P2P Worst Case - $10^4$ Block Size}
In high-contention scenarios \saSupraSTM{} performs best with 2109~ms, remaining faster than sequential, while \BSTM{} and \saBlockSTM{} reach 3012~ms and 2799~ms, nearly matching the sequential time. These results indicate that \saSupraSTM{} maintains better stability under heavy conflict, whereas other approaches suffer from rollback overheads.


\section{Block-STM: Diem vs Aptos — Code-Level Differences}

\paragraph*{Diem (\BlockSTM{})}
1. Core Repo Path: diem-core/parallel-executor \newline
2. Concurrency Engine::block\_executor: BlockSTMExecutor \newline
3. Task Execution: 	Simple Rayon-based parallel tasks \newline
4. Scheduler: Statefull \newline
5. Conflict Resolution: Naive dependency based abort/retry \newline
6. Speculative Writes: Simple MVHashMap (multi-versioned memory) \newline
7. Conflict Handling: Retry-heavy \newline
8. Performance Tuning: Minimal \newline

\paragraph*{Aptos (\BlockSTM{})}
1. Core Repo Path: aptos-core/block-executor \newline
2. Concurrency Engine: block\_executor::BlockSTMExecutor \newline
3. Task Execution: Rayon-based parallel tasks + advanced sharding and pipeline design \newline
4. Scheduler: Statefull + fine-grained dependency resolution \newline
5. Conflict Resolution: Enhanced with scheduler-dependency \STM{} \newline
6. Speculative Writes: Optimized MVHashMap with performance tuning and batching \newline
7. Conflict Handling: Smarter dependency tracking \newline
8. Performance Tuning: Extensive  \newline

\section{\BlockSTM{}: Diem vs Aptos}
Both Diem and Aptos implement a parallel execution engine based on \BlockSTM{}, a Software Transactional Memory model designed to speculatively execute transactions with potential conflicts. In Diem’s implementation, the execution model follows a relatively straightforward strategy: each transaction is executed in parallel, and after execution, a read-set validation is always performed to ensure consistency. If any of the values read during execution were overwritten by earlier transactions, the transaction is marked as having read "estimated" data and is retried. This retry-heavy approach leads to unnecessary re-executions in low-conflict workloads and lacks advanced coordination between thread.

Aptos extends and refines Diem’s Block-STM. Instead of running every task blindly in parallel, Aptos introduces execution phases (e.g., Execution, Validation) managed by a dependency-aware scheduler. When a transaction reads a speculative value, Aptos attempts to track the dependency instead of immediately retrying the transaction. This allows the runtime to delay execution until the dependency is resolved, significantly reducing wasted compute. Additionally, Aptos maintains metadata on execution status, uses adaptive concurrency control, and separates independent transactions for early commitment, all of which enhance performance and determinism in highly concurrent environments.

In isolated benchmarking of parallel execution, DiemVM performs significantly faster—typically 3× to 4× faster—than AptosVM. This difference arises from the architectural choices each system has made. DiemVM is designed for simplicity and raw throughput, invoking the MoveVM directly with minimal indirection. In contrast, AptosVM introduces additional abstraction layers, modular interfaces, and runtime tracking mechanisms that enhance flexibility, safety, and diagnostics but add overhead per transaction. Although both systems employ the Block-STM parallel execution algorithm, Aptos extends it with a more advanced scheduler, explicit phase separation (execution, validation, commit), and asynchronous task management, which improves performance under contention but slows down low-contention workloads due to task coordination and scheduling latency.

As a result, in synthetic low-conflict benchmarks such as P2P transfers, Diem’s parallel executor achieves up to 160k~tps, while Aptos’s parallel executor typically reaches around 30k~tps under the same conditions. This stark performance gap highlights the trade-off between execution speed and architectural extensibility—Diem favors lean, direct execution for speed, while Aptos prioritizes structured concurrency and system robustness.


\section{\saBlockSTM{}}
In our modified version of the Aptos Block-STM execution algorithm, we introduce a refined mechanism for identifying and processing independent transactions. Specifically, we construct a set called \Cset{}, which consists of transactions that are independent of all their preceding transactions. Independence is determined based on the absence of read-write or write-write conflicts with earlier transactions in the block.

For the transactions included in the \Cset{}, we optimize execution by skipping redundant validation steps typically performed during speculative execution. Since these transactions do not depend on any prior state changes within the block, their correctness can be established without requiring the usual conflict-checking mechanisms. This optimization not only reduces computational overhead but also improves overall throughput in high-concurrency scenarios. The remaining dependent transactions are executed and validated using the standard Block-STM pipeline to ensure consistency and correctness.

\paragraph*{Algorithm Changes }
1. Take \Cset{} as Input \newline Before execution begins, compute and supply a \Cset{} — a set of transactions that are independent of all their preceding transactions 
\begin{verbatim}
input: execute_parallel(txn_list, Cset) 
\end{verbatim}
2. Pass \Cset{} to the Scheduler \newline
Modify the scheduler interface to accept Cset as an argument.
\begin{verbatim}
scheduler = Scheduler(txn_list, \Cset{}) 
\end{verbatim}
3. Modify Validation Logic in Scheduler
Inside the scheduling loop (e.g. next\_task()), update the validation condition:
\begin{verbatim}
if validation_idx < execution_idx:
    if validation_idx in Cset:
        skip_validation()
    else:
        perform_validation()
\end{verbatim}

\section{\saSupraSTM{}}

We designed a separate DAG-based scheduler that focuses exclusively on execution of transactions. In this approach, we construct a DAG where each node represents a transaction, and edges represent dependencies based on sender-receiver relationships. This model ensures that transactions are executed only after all their dependency transactions (based on the DAG) have been completed, enabling correct ordering and maximizing parallelism.

\paragraph*{Algorithm Changes }

The function initialize\_transaction\_dependencies constructs the dependency DAG for transactions based on shared access to account addresses. It identifies which transactions depend on others by tracking which account addresses have already been accessed, and ensures that each transaction's dependencies are correctly reflected in the adjacency list and indegree counter.

\begin{verbatim}
initialize_transaction_dependencies(transactions):
    for txn_idx, accounts in transactions:
        for account in accounts:
            if account was seen before:
                add edge from parent to txn_idx
                increase indegree of txn_idx
            record latest txn_idx for account
        if indegree[txn_idx] == 0:
            push txn_idx to execution_queue
\end{verbatim}

The next\_task function is responsible for scheduling the next transaction to execute based on the current state of the execution queue and transaction statuses. It ensures that only transactions that are ready and eligible for execution are dispatched to worker threads.

\begin{verbatim}
next_task():
    if all transactions are committed:
        return Done
    if execution_queue not empty:
        txn = pop from execution_queue
        if txn is ReadyToExecute:
            mark as Executing
            return Execution(txn)
    return NoTask
\end{verbatim}

The try\_commit function finalizes the execution of a transaction by marking it as committed and propagating updates to its dependent transactions in the DAG. It plays a critical role in progressing the execution pipeline by enabling downstream transactions once their dependencies are resolved.



\begin{verbatim}
try_commit(txn_idx):
    mark txn_idx as Committed
    for child in adj_list[txn_idx]:
        decrease indegree[child]
        if indegree[child] == 0:
            push child to execution_queue
\end{verbatim}
